Expressiveness Results for an Inductive Logic of Separated Relations

In this paper we study a Separation Logic of Relations (SLR) and compare its expressiveness to (Monadic)Second Order Logic (M)SO. SLR is based on the well-known Symbolic Heap fragment of Separation Logic, whose formulae are composed of points-to assertions, inductively defined predicates, with the separating conjunction as the only logical connective. SLR generalizes the Symbolic Heap fragment by supporting general relational atoms, instead of only points-to assertions. In this paper, we restrict ourselves to finite relational structures, and hence only consider Weak (M)SO, where quantification ranges over finite sets. Our main results are that SLR and MSO are incomparable on structures of unbounded treewidth, while SLR can be embedded in SO in general. Furthermore, MSO becomes a strict subset of SLR, when the treewidth of the models is bounded by a parameter and all vertices attached to some hyperedge belong to the interpretation of a fixed unary relation symbol. We also discuss the problem of identifying a fragment of SLR that is equivalent to MSO over models of bounded treewidth.

==> draft-lipics-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}By induction on the definition of the satisfaction relation $\models _\asid $, we show that $(\universeGeneral ,\struc ) \models ^{\store }_\asid \psi \iff (\universeGeneral ',\struc ') \models ^{h \circ \store }_\asid \psi $, for any store $\store $ and any bijection $h : \universeGeneral \rightarrow \universeGeneral '$, such that, for any relation symbol $\arel \in \signature $, we have $\tuple {u_1, \ldots , u_n} \in \struc (\arel ) \iff \tuple {h(u_1), \ldots , h(u_n)} \in \struc '(\arel )$ and, for any constant $\acst \in \signature $, we have $h(\struc (\acst ))=\struc '(\acst )$. We consider the following cases: \begin {compactitem} \item $\phi = \emp $: for all $\arel \in \signature $, we have $\struc (\arel )=\emptyset \iff \struc '(\arel )=\emptyset $, by the existence of $h$. \item $\phi = \xi \sim \chi $, for $\sim \in \set {=,\neq }$: we prove only the case where $\xi \in \vars $ and $\chi \in \set {\acst _1,\ldots ,\acst _\ncst }$, the other cases being similar. By the above point, for all $\sim \in \set {=,\neq }$, by the definition of $h$, we have: \begin {compactitem} \item $\struc (\arel )=\emptyset \iff \struc '(\arel )=\emptyset $, for all $\arel \in \signature $, and \item $\store (\xi ) \sim \struc (\chi ) \iff h(\store (\xi )) \sim h(\struc (\chi )) \iff (h \circ \store )(\xi ) \sim \struc '(\chi )$. \end {compactitem} \item $\phi = \arel (\xi _1, \ldots , \xi _{\arityof {\arel }})$: $\tuple {(\struc ,\store )(\xi _1), \ldots , (\struc ,\store )(\xi _{\arityof {\arel }})} \in \struc (\arel ) \iff \langle h((\struc ,\store )(\xi _1)), \ldots , \\ h((\struc ,\store )(\xi _{\arityof {\arel }})) \rangle \in \struc '(\arel )$. If $\xi _1, \ldots , \xi _{\arityof {\arel }} \in \vars $, the latter condition is $\langle (h\circ \store )(\xi _1), \ldots , \\ (h\circ \store )(\xi _{\arityof {\arel }}) \rangle \in \struc '(\arel )$. Else, if $\xi _1, \ldots , \xi _{\arityof {\arel }} \in \set {\acst _1, \ldots , \acst _\ncst }$, the condition is $\langle h(\struc (\xi _1)), \\ \ldots , h(\struc (\xi _{\arityof {\arel }})) \rangle \in \struc '(\arel )$. The general case $\xi _1, \ldots , \xi _{\arityof {\arel }} \in \vars \cup \set {\acst _1, \ldots , \acst _\ncst }$ is a combination of the above cases. \item $\phi = \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$: this case follows by the induction hypothesis. \item $\phi = \phi _1 * \phi _2$: $\struc \models ^{\store }_\asid \phi _1 * \phi _2$ if and only if there exists disjoint and compatible structures $(\universeGeneral _1,\struc _1) \scomp (\universeGeneral _2,\struc _2) = \struc $, such that $(\universeGeneral _i,\struc _i) \models ^{\store }_\asid \phi _i$, for all $i = 1,2$. We consider the structures $(\universeGeneral '_1,\struc '_1)$ and $(\universeGeneral '_2,\struc '_2)$ as follows, for $i = 1,2$: \begin {compactitem} \item $\universeGeneral '_i = h(\universeGeneral _i)$, \item $\struc '_i(\arel ) = \set {\tuple {h(u_1), \ldots , h(u_{\arityof {\arel }})} \mid \tuple {u_1, \ldots , u_{\arityof {\arel }}} \in \struc _i(\arel )}$, for all relation symbols $\arel \in \signature $, \item $\struc '_i(\acst ) = h(\struc _i(\acst ))$, for all constant symbols $\acst \in \signature $. \end {compactitem} Then $(\universeGeneral '_1,\struc '_1)$ and $(\universeGeneral '_2,\struc '_2)$ are locally disjoint and compatible and $(\universeGeneral ',\struc ') = (\universeGeneral '_1,\struc '_1) \scomp (\universeGeneral '_2,\struc '_2)$. Moreover, by the inductive hypothesis, we have $(\universeGeneral _i,\struc '_i) \models ^{\store }_\asid \phi _i$, for all $i = 1,2$, leading to $(\universeGeneral ,\struc ') \models ^{\store }_\asid \phi _1 * \phi _2$. \item $\phi = \exists x ~.~ \psi $: by the inductive hypothesis, we obtain $(\universeGeneral ,\struc ) \models ^{\store [x\leftarrow u]}_\asid \psi \iff (\universeGeneral ',\struc ') \models ^{h\circ (\store [x\leftarrow u])}_\asid \psi \iff (\universeGeneral ',\struc ') \models ^{(h\circ \store )[x \leftarrow h(u)]}_\asid \psi \iff (\universeGeneral ',\struc ') \models ^{h\circ \store }_\asid \exists x ~.~ \psi $. \end {compactitem}\end{proof}


==> draft-lipics-pratendfive.tex <==


For a tree $\tree =(\tnodes ,\tedges ,r,\alabel )$ and a vertex $n \in \tnodes $, we denote by $\subtree {\tree }{n}$ the subtree of $\tree $ whose root is $n$. For a quantifier- and predicate-free formula $\phi $, we denote by $\phi ^n$ the formula in which every relation atom $\arel (x_1, \ldots , x_{\arityof {\arel }})$ is annotated as $\arel ^n(x_1, \ldots , x_{\arityof {\arel }})$. Atoms $\arel ^n(x_1, \ldots , x_{\arityof {\arel }})$ (and consequently formulas $\phi ^n$) have the same semantics as atoms $\arel (x_1, \ldots , x_{\arityof {\arel }})$ (resp. formulas $\phi $); these annotations serve purely as explanatory devices in our construction (Prop.~\ref {prop:slr-so}) that keep track of the node of the unfolding tree where a relation atom was introduced. \par \begin {definition}\label {def:characteristic-formula} An unfolding tree $\tree = (\tnodes ,\tedges ,r,\alabel )$ for a predicate atom $\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$ gives rise to a predicate-free formula defined inductively as follows: \[\begin {array}{l} \charform {n}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})} \isdef \\ \left (\exists y_1 \ldots \exists y_m ~.~ \psi ^r * \Asterisk _{\ell =1}^h \charform {p_\ell }{\subtree {\tree }{p_\ell }}{\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})}\right ) [x_i/\xi _i]_{i \in \interv {1}{\arityof {\apred }}} \end {array}\] such that $\alabel (r)$ is the rule: \begin {align*} \apred (x_1, \ldots , x_{\arityof {\apred }}) \leftarrow \exists y_1 \ldots \exists y_m ~.~ \psi * \Asterisk _{\ell =1}^h \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }}) \end {align*} $\psi $ is a quantifier- and predicate-free formula, and $p_1$, $\ldots $, $p_h$ are the roots of the unfolding subtrees of $\bpred _1(z_{1,1}, \ldots , z_{1,\arityof {\bpred _1}})$, $\ldots $, $\bpred _h(z_{h,1}, \ldots , z_{h,\arityof {\bpred _h}})$ in $\tree $, respectively. \end {definition} \par The unfolding trees of a predicate atom describe the set of models of that predicate atom. The following lemma is standard and we include it for self-containment reasons: \par \begin {lemma}\label {lemma:unfolding-tree} Given a structure $(\universeGeneral ,\struc )$ and store $\store $, we have $(\universeGeneral ,\struc ) \models ^\store _\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$ iff there exists an unfolding tree $\tree =(\tnodes ,\tedges ,r,\alabel )$ for $\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, such that $(\universeGeneral ,\struc ) \models ^\store \charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})}$. \end {lemma} \proof { We omit the annotations from $\phi ^n$, in this proof and simply write $\phi $ because the annotations are not relevant for this proof. ``$\Rightarrow $'' By induction on the definition of the satisfaction relation $(\universeGeneral ,\struc ) \models ^\store _\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$. Assume the relation holds because: \[(\universeGeneral ,\struc ) \models ^{\store '}_\asid \psi \overline {s} * \Asterisk _{\ell =1}^h \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}\] for a rule $\arule : \apred (x_1, \ldots , x_{\arityof {\apred }}) \leftarrow \exists y_1 \ldots \exists y_m ~.~ \psi * \Asterisk _{\ell =1}^h \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})$ from $\asid $, where $\psi $ is a quantifier- and predicate-free formula, $\overline {s} \isdef [x_1/\xi _1,\ldots ,x_{\arityof {\apred }}/\xi _{\arityof {\apred }}]$ is a substitution and $\store '$ is a store that agrees with $\store $ over $\set {\xi _1, \ldots , \xi _{\arityof {\apred }}} \cap \vars $. Then there exist structures $(\universeGeneral _0,\struc _0) \scomp \ldots \scomp (\universeGeneral _h,\struc _h) = (\universeGeneral ,\struc )$, such that $(\universeGeneral _0,\struc _0) \models ^{\store '} \psi \overline {s}$ and $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '}_\asid \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}$, for all $\ell \in \interv {1}{h}$. By the induction hypothesis, there exist unfolding trees $\tree _\ell = (\tnodes _\ell ,\tedges _\ell ,r_\ell ,\alabel _\ell )$ for $\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}$, such that $(\universeGeneral _\ell ,\struc _\ell ) \models _\asid ^{\store '} \charform {r_\ell }{\tree _\ell }{\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}}$, for all $\ell \in \interv {1}{h}$. Then $\tree = (\tnodes ,\tedges ,r,\alabel )$ is defined as $\tnodes \isdef \set {r} \cup \bigcup _{\ell =1}^h \tnodes _\ell $, $\tedges \isdef \set {(r,r_\ell ) \mid \ell \in \interv {1}{h}} \cup \bigcup _{\ell =1}^h \tedges _\ell $ and $\alabel = \set {(r,\arule )} \cup \bigcup _{\ell =1}^h \alabel _\ell $, assuming w.l.o.g. that $\tnodes _\ell \cap \tnodes _k = \emptyset $, for all $1 \leq \ell < k \leq h$ and $r \not \in \bigcup _{\ell =1}^h\tnodes _\ell $. The check that $(\universeGeneral ,\struc ) \models ^\store \charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})}$ is routine. \par \vspace *{\baselineskip } \noindent ''$\Leftarrow $'' By induction on the structure of $\tree $. Let $p_1, \ldots , p_h$ be the children of $r$ in $\tree $. By Def. \ref {def:unfolding-tree}, we have: \[((\universeGeneral ,\struc ) \models ^{\store '} \psi \overline {s} * \Asterisk _{\ell =1}^h \charform {p_\ell }{\subtree {\tree }{p_\ell }}{\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})}\overline {s}\] where $\overline {s}\isdef [x_1/\xi _1,\ldots ,x_{\arityof {\apred }}/\xi _{\arityof {\apred }}]$ is a substitution, $\store '$ is a store that agrees with $\store $ over $\set {\xi _1, \ldots , \xi _{\arityof {\apred }}} \cap \vars $ and $\alabel (r)=\apred (x_1, \ldots , x_{\arityof {\apred }}) \leftarrow \exists y_1 \ldots \exists y_m ~.~ \psi * \Asterisk _{\ell =1}^h \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})$ is a rule from $\asid $. Then there exist structures $(\universeGeneral _0,\struc _0) \scomp \ldots \scomp (\universeGeneral _h,\struc _h) = (\universeGeneral ,\struc )$, such that $(\universeGeneral _0,\struc _0) \models ^{\store '} \psi \overline {s}$ and $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '} \charform {p_\ell }{\proj {\tree }{p_\ell }}{\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})}\overline {s}$, for all $\ell \in \interv {1}{h}$. Since $\subtree {\tree }{p_\ell }$ is an unfolding tree for $\bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}$, by the inductive hypothesis, we obtain $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '}_\asid \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}$, for all $\ell \in \interv {1}{h}$. Then, we have $(\universeGeneral ,\struc ) \models ^{\store '}_\asid \psi \overline {s} * \Asterisk _{\ell =1}^h \bpred _\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred _\ell }})\overline {s}$, leading to $(\universeGeneral ,\struc ) \models ^{\store }_\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$. \qed } \par \vspace *{\baselineskip }\noindent The formul{\ae } from the definition of $\mathfrak {F}$ are given below:

\vspace *{\baselineskip } {\raggedright (\text {\ref {it2:slr-so}})} $\begin {array}{l} \bigwedge _{i \in \interv {1}{\nrule }} \bigwedge _{\arel _k \text { occurs in } \arule _i} \forall y ~.~ X_i(y) \rightarrow \exists z_1 \ldots \exists z_{\arityof {\arel _k}} ~.~ \arel _k(z_1,\ldots , z_{\arityof {\arel _k}}) \wedge \bigwedge _{\ell \in \interv {1}{\arityof {\arel _k}}} Z_{k,\ell }(y,z_\ell ) \end {array}$

\vspace *{\baselineskip } {\raggedright (\text {\ref {it3:slr-so}})} $\begin {array}{l} \bigwedge _{i, j \in \interv {1}{\nrule }} \bigwedge _{\arel _k \text { occurs in } \arule _i, \arule _j} \forall y \forall y' \forall z_1 \forall z'_1 \ldots \forall z_{\arityof {\arel _k}} \forall z'_{\arityof {\arel _k}} ~.~ \\ \Big (y \neq y' \wedge X_i(y) \wedge X_j(y') \wedge \bigwedge _{\ell \in \interv {1}{\arityof {\arel _k}}} (Z_{k,\ell }(y,z_\ell ) \wedge Z_{k,\ell }(y',z'_\ell ))\Big ) \rightarrow \bigvee _{\ell \in \interv {1}{\arityof {\arel _k}}} z_\ell \neq z'_\ell \end {array}$

\vspace *{\baselineskip } {\raggedright (\text {\ref {it4:slr-so}})} $\begin {array}{l} \bigwedge _{k \in \interv {1}{\nrel }}\forall z_1 \ldots \forall z_{\arityof {\arel _k}} ~.~ \arel _k(z_1, \ldots , z_{\arityof {\arel _k}}) \rightarrow \\ \exists y ~.~ \bigvee _{\arel _k \text { occurs in } \arule _i} \big (X_i(y) ~\wedge \bigwedge _{\ell \in \interv {1}{\arityof {\arel _k}}} Z_{k,\ell }(y,z_\ell )\big ) \end {array}$

\vspace *{\baselineskip } {\raggedright (\text {\ref {it5:slr-so}})} $\begin {array}{l} \bigwedge _{k,\ell \in \interv {1}{\nrel }} \bigwedge _{\begin {array}{l} \scriptstyle {\arel _k \text { occurs in } \arule _i} \\[-1mm] \scriptstyle {\arel _\ell \text { occurs in } \arule _j} \end {array}} \bigwedge _{m \in \interv {1}{\arityof {\arel _k}}} \bigwedge _{n \in \interv {1}{\arityof {\arel _\ell }}} \forall y \forall y' \forall z' \forall z' ~.~ \\ \big (X_i(y) \wedge X_j(y') \wedge \mathit {isEq}_{k,\ell ,m,n}(y, y', \set {X_i}_{i=1}^\nrule , \set {Y_j}_{j=1}^\npred ) \wedge ~ Z_{k,m}(y,z) \wedge Z_{\ell ,n}(y',z')\big ) \rightarrow z = z' \end {array}$ \par \vspace *{\baselineskip }\noindent The formula $\mathit {isEq}_{k,\ell ,m,n}(y,y',\set {X_i}_{i=1}^\nrule ,\set {Y_j}_{j=1}^\npred )$ asserts that there is a path in the unfolding tree between the store values (i.e., vertices of the tree) of $y$ and $y'$, such that the $m$-th and $n$-th variables of the relation atoms $\arel _k(z_1, \ldots , z_{\arityof {\arel _k}})$ and $\arel _\ell (z'_1, \ldots , z'_{\arityof {\arel _\ell }})$ occurring in the labels of the vertices $y$ and $y'$, respectively, are bound to the same value.

\vspace *{\baselineskip } {\raggedright (\text {\ref {it6:slr-so}})} $\begin {array}{l} \bigwedge _{\xi \neq \chi \text { occurs in } \arule _i} \bigwedge _{k,\ell \in \interv {1}{\nrel }} \bigwedge _{\begin {array}{l} \scriptstyle {\arel _{k} \text { occurs in } \arule _{j_k}} \\ \scriptstyle {\arel _{\ell } \text { occurs in } \arule _{j_\ell }} \end {array}} \bigwedge _{r \in \interv {1}{\arityof {\arel _k}}} \bigwedge _{s\in \interv {1}{\arityof {\arel _\ell }}} \\ \forall y \forall y' \forall y'' \forall z' \forall z'' . \Big (X_i(y) \wedge X_{j_k}(y') \wedge X_{j_\ell }(y'') \wedge Z_{k,r}(y',z') ~\wedge \\ Z_{\ell ,s}(y'',z'') \wedge \mathit {varEq}_{\xi ,k,r}(y, y', \set {X_i}_{i=1}^N, \set {Y_j}_{j=1}^M) ~\wedge \mathit {varEq}_{\chi ,\ell ,s}(y, y'', \set {X_i}_{i=1}^N)\Big ) \rightarrow z' \neq z'' \end {array}$ \par \vspace *{\baselineskip }\noindent The formula $\mathit {varEq}_{\xi ,k,r}(x,y,\set {X_i}_{i=1}^\nrule ,\set {Y_j}_{j=1}^\npred )$ states that the variable $\xi $ occurring in the label of the unfolding tree vertex $x$ is bound to the variable $z_r$ that occurs in a relation atom $\arel _k(z_1, \ldots , z_{\arityof {\arel _i}})$ in the label of the vertex $y$.

\vspace *{\baselineskip } {\raggedright (\text {\ref {it7:slr-so}})} $\begin {array}{l} \bigwedge _{\arule _i \text { defines } \apred } \bigwedge _{j \in \interv {1}{\arityof {\apred }}} \forall y \forall z ~.~ \\ \Big (X_i(x) \wedge \mathit {varEq}_{\xi _j,k,r}(x, y, \set {X_i}_{i=1}^\nrule ,\set {Y_j}_{j=1}^\npred ) \wedge Z_{k,r}(y,z)\Big ) \rightarrow \xi _j = z \end {array}$

\noindent The above formul{\ae } $\mathit {isEq}_{k,\ell ,m,n}(x,y,\set {X_i}_{i=1}^\nrule ,\set {Y_j}_{j=1}^\npred )$ and $\mathit {varEq}_{\xi ,k,r}(x,y,\set {X_i}_{i=1}^\nrule ,\set {Y_j}_{j=1}^\npred )$ can be written in \mso , using standard tree automata construction techniques, similar to the definition of \mso \ formul{\ae } that track parameters in an unfolding tree for \seplog , with edges definable by \mso \ formul{\ae } over the signature of \seplog \ \cite {DBLP:conf/cade/IosifRS13}.

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}``$\Rightarrow $'' By Lemma \ref {lemma:unfolding-tree}, there exists an unfolding tree $\tree = (\tnodes ,\tedges ,r,\alabel )$ of $\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, such that $(\universeGeneral ,\struc ) \models ^{\store } \charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})}$. Let $\charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})} = \exists y_1 \ldots \exists y_K ~.~ \Phi $, where $\Phi $ is a quantifier- and predicate-free formula. Note that, by Def. \ref {def:unfolding-tree}, no second order variables occur in $\charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})}$. Hence there exists a store $\store '$ that agrees with $\store $ over $\xi _1, \ldots , \xi _{\arityof {\apred }}$, such that $(\universeGeneral ,\struc ) \models ^{\store '} \Phi $. We define another store $\store ''$, that agrees with $\store $ and $\store '$ over $\xi _1, \ldots , \xi _{\arityof {\apred }}$ such that, moreover, we have: \begin {compactitem} \item $\store ''(x)=r$, \item $\store ''(X_i) = \set {n \in \tnodes \mid \alabel (n) = \arule _i}$, for all $i \in \interv {1}{\nrule }$, \item $\store ''(Y_j) = \set {(n,m) \in \tnodes \times \tnodes \mid m \text { is the $j$-th child of } n}$, for all $j \in \interv {1}{\npred }$; we consider that the order between the children of a vertex in an unfolding tree is the syntactic order of their corresponding predicate atoms, in the sense of Def. \ref {def:unfolding-tree}, \item $\store ''(Z_{k,\ell }) = \{(n,(\struc ,\store ')(\xi _\ell )) \mid n \in \tnodes ,~ \arel ^n_k(\xi _1,\ldots ,\xi _{\arityof {\arel _k}}) \\ \text { occurs in } \Phi \}$, for all $k \in \interv {1}{\nrel }$ and $\ell \in \interv {1}{\arityof {\arel _k}}$. \end {compactitem} We have $(\universeGeneral ,\struc ) \Models ^{\store ''} \mathfrak {T}(x, \set {X_i}_{i=1}^\nrule , \set {Y_j}_{j=1}^\npred )$ because $\tree $ is an unfolding tree for $\apred (\xi _1,\ldots ,\xi _{\arityof {\apred }})$, by Def. \ref {def:unfolding-tree}. The proof of \((\universeGeneral ,\struc ) \Models ^{\store ''} \mathfrak {F}(\xi _1, \ldots , \xi _{\arityof {\apred }},x, \set {X_i}_{i=1}^\nrule , \set {Y_j}_{j=1}^\npred , \set {\set {Z_{k,\ell }}_{\ell =1}^{\arityof {\arel _k}}}_{k=1}^\nrel )\) follows from $(\universeGeneral ,\struc )\models ^{\store '} \Phi $ and the definition of $\store ''$, by the points (\ref {it1:slr-so}-\ref {it7:slr-so}) from the definition of $\mathfrak {F}$. We obtain $(\universeGeneral ,\struc ) \Models ^{\store } \mathfrak {A}^\apred _\asid (\xi _1, \ldots , \xi _{\arityof {\apred }})$ from the definition of $\mathfrak {A}^\apred _\asid $. \par \noindent ''$\Leftarrow $'' There exists a store $\store '$ that agrees with $\store $ over $\xi _1, \ldots , \xi _{\arityof {\apred }}$, such that: \begin {align} (\universeGeneral ,\struc ) \Models ^{\store '} & \mathfrak {T}(x, \set {X_i}_{i=1}^\nrule , \set {Y_j}_{j=1}^\npred ) \label {eq:tree} \\ (\universeGeneral ,\struc ) \Models ^{\store '} & \mathfrak {F}(\xi _1, \ldots , \xi _{\arityof {\apred }},x, \set {X_i}_{i=1}^\nrule , \set {Y_j}_{j=1}^\npred , \set {\set {Z_{k,\ell }}_{\ell =1}^{\arityof {\arel _k}}}_{k=1}^\nrel ) \label {eq:form} \end {align} By (\ref {eq:tree}) we obtain an unfolding tree $\tree = (\tnodes ,\tedges ,r,\alabel )$ for $\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, such that: \begin {compactitem} \item $\tnodes = \bigcup _{i=1}^\nrule \store '(X_i)$, \item $\tedges = \bigcup _{j=1}^\npred \store '(Y_j)$, \item $\alabel (n) = \arule _i \iff n \in \store '(X_i)$, for all $n \in \tnodes $ and $i \in \interv {1}{\nrule }$. \end {compactitem} Let $\charform {r}{\tree }{\apred (\xi _1, \ldots , \xi _{\arityof {\apred }})} = \exists y_1 \ldots \exists y_K ~.~ \Phi $, where $\Phi $ is a quantifier- and predicate-free formula (Def. \ref {def:unfolding-tree}). By Lemma \ref {lemma:unfolding-tree}, it is sufficient to show the existence of a store $\store ''$ that agrees with $\store $ over $\xi _1, \ldots , \xi _{\arityof {\apred }}$, such that $(\universeGeneral ,\struc ) \models ^{\store ''} \Phi $. Let $f_{k,\ell }$ denote the partial mapping defined by $\store '(Z_{k,\ell })$, for each $k \in \interv {1}{\nrel }$ and $\ell \in \interv {1}{\arityof {\arel }}$, by point (\ref {it1:slr-so}) of the definition of $\mathfrak {F}$. For each $r \in \interv {1}{K}$, we define $\store ''(y_r) \isdef f_{k,\ell }(n)$ if $y_r$ occurs in or is constrained to be equal to a term $\xi _\ell $ that occurs in an annotated relation atom $\arel ^n_k(\xi _1, \ldots , \xi _{\arityof {\arel _k}})$ from $\Phi $. Note that there can be at most one such relation atom in $\Phi $, because of the assumption that in each rule from $\asid $ at most one relation atom $\arel _k(z_1,\ldots ,z_{\arityof {\arel _k}})$ occurs. Otherwise, if $y_r$ is not constrained in $\Phi $ to be equal to a term that occurs in a relation atom, $\store ''(y_r)$ is given an arbitrary fresh value. Because the equalities and disequalities from $\Phi $ are taken care of by points (\ref {it5:slr-so}) and (\ref {it6:slr-so}) from the definition of $\mathfrak {F}$, it remains to check the satisfaction of the relation atoms from $\Phi $. To this end, we define a decomposition $(\universeGeneral ,\struc ) = \bigscomp _{n \in \tnodes ,~ k \in \interv {1}{N}} (\universeGeneral _{n,k},\struc _{n,k})$ such that $(\universeGeneral _{n,k},\struc _{n,k}) \models ^{\store ''} \arel _k(\xi _1,\ldots ,\xi _{\arityof {\arel _k}})$, for all relation atoms $\arel _k^n(\xi _1,\ldots ,\xi _{\arityof {\arel _k}})$ from $\Phi $. Such a decomposition is possible due to points (\ref {it2:slr-so}-\ref {it4:slr-so}) from the definition of $\mathfrak {F}$.\end{proof}


==> draft-lipics-pratendfour.tex <==


\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Let $\asid $ be an SID. For each predicate $\apred $ defined by a rule in $\asid $ and each partition $I_1, \ldots , I_k$ of $\interv {1}{\arityof {\apred }}$, we consider a fresh predicate $\apred _{I_1,\ldots ,I_k}$ of arity $k\geq 1$, not occurring in $\asid $. Let $\asid '$ be the SID obtained from $\asid $ by introducing, for each rule: \[\begin {array}{l} \apred (x_1, \ldots , x_{\arityof {\apred }}) \leftarrow \exists y_1 \ldots \exists y_m ~.~ \phi * \Asterisk _{\ell =1}^h \bpred ^\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred ^\ell }}) \in \asid ~~(\dagger ) \end {array}\] where $\phi $ is a quantifier- and predicate-free formula and for each equivalence relation $\approx $ on the set of variables $\set {x_1, \ldots , x_{\arityof {\apred }}} \cup \set {y_1,\ldots ,y_m}$ that is compatible with all equalities in $\phi $, i.e., $x = y$ occurs in $\phi $ only if $x \approx y$, the following rules: \[\begin {array}{ll} \apred _{I_1,\ldots ,I_k}(x_1, \ldots , x_k) \leftarrow \\ \hspace *{5mm} \big (\exists y_{j_1} \ldots \exists y_{j_n} ~.~ \psi ~* \Asterisk _{\ell =1}^k \bpred ^\ell _{J^\ell _1,\ldots ,J^\ell _{s^\ell }}(z_{r_{\ell ,1}}, \ldots ,z_{r_{\ell ,s^\ell }})\big )[x_{i_1}/x_1, \ldots , x_{i_k}/x_k] & (\ddagger ) \\[1mm] \apred (x_1, \ldots , x_{\arityof {\apred }}) \leftarrow ~\apred _{I_1,\ldots ,I_k}(x_{i_1}, \ldots , x_{i_k}) & (\star ) \end {array}\] where: \begin {compactitem} \item $\approx $ induces the partitions $I_1, \ldots , I_k$ of $\interv {1}{\arityof {\apred }}$ and $J^\ell _1, \ldots , J^\ell _{s^\ell }$ of $\interv {1}{\arityof {\bpred ^\ell }}$, for each $\ell \in \interv {1}{k}$, \item $x_{i_j}$ and $z_{r_{\ell ,s^\ell }}$ are the first in their $\approx $-equivalence classes, respectively, in the total order $x_1 < \ldots < x_{\arityof {\apred }} < y_1 < \ldots < y_m$, \item $\psi $ is obtained from $\phi $ by replacing each variable $x$, such that $x \approx x_{i_j}$ with $x_{i_j}$, respectively each $z$, such that $z \approx z_{r_{\ell ,s^j}}$ with $z_{r_{\ell ,s^j}}$, and replacing the trivial equalities of the form $x = x$ by $\emp $, \item the quantifier prefix $\exists y_{j_1} \ldots \exists y_{j_n}$ is the result of eliminating from $\exists y_1 \ldots \exists y_m$ the variables that do not occur in $\fv {\psi } \cup \bigcup _{\ell =1}^h \set {z_{\ell ,r_1}, \ldots , z_{r_{\ell ,s^\ell }}}$. \end {compactitem} In particular, one can remove from $\asid '$ the rules containing unsatisfiable disequalities of the form $x \neq x$, obtained from the above transformations. We are left with proving the equivalence from the statement. \par \noindent ``$\Rightarrow $'' Assume that $(\universeGeneral ,\struc ) \models ^\store _\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$ for a store $\store $, and let $\approx $ be the equivalence relation over $\set {\xi _1, \ldots , \xi _{\arityof {\apred }}}$, defined as $\xi _i \approx \xi _j \iff (\struc ,\store )(\xi _i) = (\struc ,\store ) (\xi _j)$. We now prove by induction that $(\universeGeneral ,\struc ) \models ^\store _\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$ implies $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred _{I_1, \ldots , I_k}(\xi _{i_1}, \ldots , \xi _{i_k})$, where $\set {I_1, \ldots , I_k}$ is the partition of $\interv {1}{\arityof {\apred }}$ induced by $\approx $ and the $\xi _{i_j}$ are minimal representatives of $I_j$ in some fixed total order. Since $(\universeGeneral ,\struc ) \models ^\store _\asid \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, there is a rule ($\dagger $) in $\asid $, a store $\store '$, that agrees with $\store $ over $\xi _{1}, \ldots , \xi _{\arityof {\apred }}$ and structures $(\universeGeneral _0,\struc _0) \scomp \ldots \scomp (\universeGeneral _h,\struc _h) = (\universeGeneral ,\struc )$, such that $(\universeGeneral _0,\struc _0) \models ^{\store '} \phi \overline {s}$ and $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '}_\asid \bpred ^\ell (z_{\ell ,1},\ldots ,z_{\ell ,\arityof {\bpred ^\ell }})\overline {s}$, for all $\ell \in \interv {1}{h}$, where $\overline {s} \isdef [x_{1}/\xi _{1}, \ldots , x_{n}/\xi _{n}]$ is the substitution that replaces the formal parameters by terms. Let $\approx '$ be the equivalence over $x_1 < \ldots < x_{\arityof {\apred }} < y_1 < \ldots < y_m$ defined as $x \approx y \iff \store '(x) = \store '(y)$. By the inductive hypothesis, we have $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '}_{\asid '} \bpred ^\ell _{J_1, \ldots , r_{s^\ell }}(z_{J_{\ell ,1}},\ldots ,z_{r_{\ell ,s^\ell }})\overline {s}$, where $z_{r_{\ell ,1}},\ldots ,z_{r_{\ell ,s^\ell }}$ is the sequence of minimal representatives wrt $\approx '$. Since $\approx ' \ \supseteq \ \approx $, there exists a rule of type ($\ddagger $) in $\asid '$ allowing to infer that $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred _{I_1, \ldots , I_k}(\xi _{i_1}, \ldots , \xi _{i_k})$. We finally obtain $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, by a rule of type ($\star $). \par \noindent ''$\Leftarrow $'' Assume that $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$. Then, by a rule of type ($\star $) from $\asid '$, we must have $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred _{I_1, \ldots , I_k}(\xi _{i_1}, \ldots , \xi _{i_k})$. We now prove by induction that $(\universeGeneral ,\struc ) \models ^\store _{\asid '} \apred _{I_1, \ldots , I_k}(\xi _{i_1}, \ldots , \xi _{i_k})$ implies that $(\universeGeneral ,\struc ) \models ^{\store '}_{\asid } \apred (\xi _1, \ldots , \xi _{\arityof {\apred }})$, where $\store '$ is a store that maps each $\xi _j \in \vars $, such that $j \in I_j$, into $(\struc ,\store )(\xi _{i_j})$. Let $(\universeGeneral ,\struc ) \models ^{\store ''}_{\asid '} (\psi * \Asterisk _{\ell =1}^h \bpred ^\ell _{J^\ell _1,\ldots ,J^\ell _{s^\ell }}(z_{r_{\ell ,1}}, \ldots , z_{r_{\ell ,s^\ell }}))\overline {s}$ by a rule of type ($\ddagger $), where $\store ''$ is a store that agrees with $\store $ over $\xi _{i_1}, \ldots , \xi _{i_k}$ and $\overline {s} \isdef [x_1/\xi _{i_1}, \ldots , x_k/\xi _{i_k}]$ is a substitution. Then there exists structures $(\universeGeneral _0,\struc _0) \scomp \ldots \scomp (\universeGeneral _h,\struc _h) = (\universeGeneral ,\struc )$, such that $(\universeGeneral _0,\struc _0) \models ^{\store ''} \psi \overline {s}$ and $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store ''}_{\asid '} \bpred ^\ell _{J^\ell _1,\ldots ,J^\ell _{s^\ell }}(z_{r_{\ell ,1}}, \ldots , z_{r_{\ell ,s^\ell }})\overline {s}$, for all $\ell \in \interv {1}{h}$. By the definition of $\asid '$, there exists a rule of type ($\dagger $) in $\asid $ and a corresponding equivalence relation $\approx $ over $x_1 < \ldots < x_{\arityof {\apred }} < y_1 < \ldots < y_m$, which induces the partitions $\set {I_1, \ldots , I_k}$ of $\interv {1}{\arityof {\apred }}$ and $\set {J^\ell _1, \ldots , J^\ell _{s^\ell }}$ of $\interv {1}{\arityof {\bpred ^\ell }}$, for each $\ell \in \interv {1}{k}$, and $x_{i_j}$ and $z_{r_{\ell ,s^\ell }}$ are the first in their $\approx $-equivalence classes. We can now choose a store $\store '''$, such that: \begin {compactitem} \item $(\struc ,\store ''')(\xi _j) = (\struc ,\store '')(\xi _{i_j})$, for all $j \in \interv {1}{k}$, and \item $(\struc ,\store ''')(z_j\overline {s}) = (\struc ,\store '')(z_{r_{\ell ,q}}\overline {s})$ if $j \in J^\ell _q$, for all $\ell \in \interv {1}{h}$ and $q \in \interv {1}{s^\ell }$. \end {compactitem} By the definition of $\psi $, we have $(\universeGeneral _0,\struc _0) \models ^{\store '''} \phi $. By the inductive hypothesis, we obtain $(\universeGeneral _\ell ,\struc _\ell ) \models ^{\store '''}_\asid \bpred ^\ell (z_{\ell ,1}, \ldots , z_{\ell ,\arityof {\bpred ^\ell }})$, for all $\ell \in \interv {1}{h}$. Hence $(\universeGeneral ,\struc ) \models ^{\store '''}_\asid \apred (\xi _1,\ldots ,\xi _{\arityof {\apred }})$, by a rule of type ($\dagger $).\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}The structure $(\universeGeneral ,\overline {\struc })$ is built inductively on the definition of the satisfaction relation $(\universeGeneral ,\struc ) \models ^{\store }_\asid \apred (x_1,\ldots ,x_{\arityof {\apred }})$. Since no existentially quantified variable is constrained by equality during this derivation, one can use the definition of $\imodels {\store }{\asid }{}$ instead, thus ensuring that $(\universeGeneral ,\overline {\struc }) \imodels {\store }{\asid }{} \apred (x_1,\ldots ,x_{\arityof {\apred }})$. Moreover, since the values of the existentially quantified variables are pairwise distinct in $(\universeGeneral ,\overline {\struc })$, there are only finitely many non-isomorphic structures $(\universeGeneral ,\struc ')$, such that $\overline {\struc '} = \overline {\struc }$.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Let $W$ be the maximal number of variables that occur free or bound in a rule from $\asid $. We build a tree decomposition $\tree = (\tnodes ,\tedges ,r,\alabel )$ of $(\universeGeneral ,\struc )$, such that $\bigcup _{n \in \tnodes } \alabel (n) \subseteq \universeGeneral $, inductively on the definition of the satisfaction relation $(\universeGeneral ,\struc ) \imodels {\store }{\asid }{} \apred (\xi _1,\ldots ,\xi _{\arityof {\apred }})$. Assume that $(\universeGeneral ,\struc ) \imodels {\store }{\asid }{} \apred (\xi _1,\ldots ,\xi _{\arityof {\apred }})$ is the consequence of a rule $\apred (x_1,\ldots ,x_{\arityof {\apred }}) \leftarrow \exists y_1 \ldots \exists y_m ~.~ \psi * \Asterisk _{\ell =1}^k \bpred _\ell (z^\ell _1, \ldots , z^\ell _{\arityof {\bpred _\ell }})$ from $\asid $, where $\psi $ is a quantifier- and predicate-free formula, such that \((\universeGeneral ,\struc ) \imodels {\store '}{\asid }{} \exists y_1 \ldots \exists y_m ~.~ \psi * \Asterisk _{\ell =1}^k \bpred _\ell (z^\ell _1, \ldots , z^\ell _{\arityof {\bpred _\ell }})\) and $\store '(x_i)=(\struc ,\store )(\xi _i)$, for all $i \in \interv {1}{\arityof {\apred }}$. Then there exists a store $\store ''$ that agrees with $\store '$ over $x_1, \ldots , x_{\arityof {\apred }}$, such that $\store ''(y_1), \ldots , \store ''(y_m)$ are pairwise distinct, and structures $(\universeGeneral _0,\struc _0) \scomp \ldots \scomp (\universeGeneral _k,\struc _k) = (\universeGeneral ,\struc )$, such that: \begin {compactitem} \item $\universeGeneral _0 \cap \universeGeneral _\ell = \store ''(\fv {\psi } \cap \set {z_1^\ell , \ldots , z_{\arityof {\bpred _\ell }}^\ell })$, for all $\ell \in \interv {1}{k}$, \item $\universeGeneral _i \cap \universeGeneral _j = \store ''(\set {z_1^i, \ldots , z_{\arityof {\bpred _i}}^i} \cap \set {z_1^j, \ldots , z_{\arityof {\bpred _j}}^j})$, for all $1 \leq i < j \leq k$, \item $(\universeGeneral _0,\struc _0) \models ^{\store ''} \psi $, and \item $(\universeGeneral _\ell ,\struc _\ell ) \imodels {\store ''}{\asid }{} \bpred _\ell (z^\ell _1, \ldots , z^\ell _{\arityof {\bpred _\ell }})$, for all $\ell \in \interv {1}{k}$. \end {compactitem} By the inductive hypothesis, there exists a tree decomposition $\tree _\ell = (\tnodes _\ell ,\tedges _\ell ,r_\ell ,\alabel _\ell )$ of $\struc _\ell $, such that $\twof {\tree _\ell } \leq W$ and $\bigcup _{n \in \tnodes _\ell } \alabel (n) \subseteq \universeGeneral _\ell $, for each $\ell \in \interv {1}{k}$. We define the tree decomposition $\tree = (\tnodes ,\tedges ,r,\alabel )$ such that $\tree _1, \ldots , \tree _k$ are the immediate subtrees of the root and $\alabel (r)=\set {\store ''(x_1), \ldots , \store ''(x_{\arityof {\apred }})} \cup \set {\store ''(y_1), \ldots , \store ''(y_m)}$. Then, for each relation atom $\arel (z_1,\ldots ,z_{\arityof {\arel }})$ that occurs in $\psi $, the set $\set {\store ''(z_1), \ldots , \store ''(z_{\arityof {\arel }})}$ is a subset of the label of the root, thus fulfilling point (\ref {it1:treewidth}) of Def. \ref {def:treewidth}. To check point (\ref {it2:treewidth}) of Def. \ref {def:treewidth}, let $u \in \alabel _i(n_i) \cap \alabel _j(n_j)$, where $n_i \in \tnodes _i$ and $n_j \in \tnodes _j$, for some $1 \leq i < j \leq k$. Since $(\universeGeneral _i,\struc _i) \imodels {\store ''}{\asid }{} \bpred _i(z^i_1,\ldots ,z^i_{\arityof {\bpred _i}})$, $(\universeGeneral _j,\struc _j) \imodels {\store ''}{\asid }{} \bpred _j(z^j_1,\ldots ,z^j_{\arityof {\bpred _j}})$ and $\universeGeneral _i \cap \universeGeneral _j = \store ''(\set {z_1^i, \ldots , z_{\arityof {\bpred _i}}^i} \cap \set {z_1^j, \ldots , z_{\arityof {\bpred _j}}^j})$, we obtain that $u$ is not the image of an existentially quantified variable via $\store ''$, hence $u = \store ''(z)$, for some $z \in \set {z^i_1,\ldots ,z^i_{\arityof {\bpred _i}}} \cap \set {z^j_1,\ldots ,z^j_{\arityof {\bpred _j}}} \subseteq \set {\xi _1, \ldots , \xi _{\arityof {\apred }}} \cup \set {y_1, \ldots , y_m}$. Then $u \in \alabel (r)$, thus fulfilling point (\ref {it2:treewidth}) of Def. \ref {def:treewidth}. We have $\twof {\tree } = \max \set {\cardof {\alabel (r)}-1, \twof {\tree _1}, \ldots , \twof {\tree _k}} \leq W$, since $\cardof {\alabel (r)} \leq \arityof {\apred }+m \leq W$, by the definition of $\alabel (r)$, and $\twof {\tree _i} \leq W$, for all $i \in \interv {1}{k}$, by the inductive hypothesis.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\asid '_\phi $ be the normalized SID, such that $(\universeGeneral ,\struc ) \models _{\asid '_\phi } \apred _\phi ()$, by Lemma \ref {lemma:normalized-sid}. Then, there exists a structure $(\universeGeneral ,\overline {\struc })$ and a store $\store $, such that $(\universeGeneral ,\overline {\struc }) \imodels {\store }{\asid '_\phi }{} \apred _\phi ()$, by Lemma \ref {lemma:injective-model}. By Lemma \ref {lemma:injective-bounded}, we also obtain $\twof {\universeGeneral ,\overline {\struc }} \leq W$, where $W$ depends only of $\asid '_\phi $ and hence of $\asid $ and $\phi $. If $\apred _\phi ()$ has finitely many non-isomorphic models, there is nothing to prove. Otherwise, consider an infinite sequence $(\universeGeneral _1,\struc _1), (\universeGeneral _2,\struc _2), \ldots $ of non-isomorphic models of $\apred _\phi ()$. Since, by Lemma \ref {lemma:injective-model}, for any given $i\geq 1$ there are only finitely many non-isomorphic structures $(\universeGeneral _j,\struc _j)$, such that $\overline {\struc }_i = \overline {\struc }_j$, there exists an infinite subsequence $(\universeGeneral _{i_1},\struc _{i_1}), (\universeGeneral _{i_2},\struc _{i_2}), \ldots $, such that $\twof {\universeGeneral _{i_j},\struc _{i_j}} \leq W$, for all $j \geq 1$.\end{proof}


==> draft-lipics-pratendsix.tex <==


We consider tree decompositions of a special form and show that this restriction does not lose generality (see Lemma~\ref {lemma:reduced-tree-decompositions} below). \par \begin {definition}\label {def:reduced-td} A tree decomposition $\tree =(\tnodes ,\tedges ,r,\alabel )$ of a structure $(\universeGeneral ,\struc )$ is said to be \emph {reduced} iff the following hold: \begin {compactenum} \item \label {it1:reduced-td} for each $\arel \in \signature $ and each $\tuple {u_1, \ldots , u_{\arityof {\arel }}} \in \struc (\arel )$ there exists a leaf $n \in \tnodes $ such that $\set {u_1, \ldots , u_{\arityof {\arel }}} \subseteq \alabel (n)$, called the \emph {witness} of $\tuple {u_1, \ldots , u_{\arityof {\arel }}} \in \struc (\arel )$, \item \label {it2:reduced-td} a leaf witnesses exactly one tuple $\tuple {u_1, \ldots , u_{\arityof {\arel }}} \in \struc (\arel )$, \item \label {it3:reduced-td} each node in $\tree $ has at most two children, \item \label {it4:reduced-td} if $n \in \tnodes $ has two children $m_1,m_2 \in \tnodes $ then $\alabel (n) = \alabel (m_1) = \alabel (m_2)$, \item \label {it6:reduced-td} $\cardof {\alabel (n)} = k+1$, for all $n \in \tnodes $. \item \label {it5:reduced-td} if $n \in \tnodes $ has one child $m \in \tnodes $ then either $\alabel (n) = \alabel (m)$ or we have $\cardof {\alabel (n) \setminus \alabel (m)} = \cardof {\alabel (m) \setminus \alabel (n)} = 1$. \end {compactenum} \end {definition} \par \begin {lemma}\label {lemma:reduced-tree-decompositions} A structure $(\universeGeneral ,\struc )$ has a tree decomposition of width $k$ iff it has a reduced tree decomposition of width $k$. \end {lemma} \proof { Let $\tree =(\tnodes ,\tedges ,r,\alabel )$ be the original tree decomposition. We perform the following actions, corresponding to the cases from Def. \ref {def:reduced-td}, in this order: \begin {compactitem} \item [(\ref {it1:reduced-td})] For each non-leaf node $n_0\in \tnodes $, witnessing a tuple $\tuple {u_1, \ldots , u_{\arityof {\arel }}} \in \struc (\arel )$, we add a leaf $m_1$ directly to $n_0$, labeled with $\alabel (n_0)$. \item [(\ref {it2:reduced-td})] for each leaf $n_0\in \tnodes $, that witnesses $k\geq 2$ tuples, we append $k$ children $m_1, \ldots , m_k$, each labeled by $\alabel (n_0)$. \item [(\ref {it3:reduced-td})] Let $n_0 \in \tnodes $ be a node with children $n_1, \ldots , n_\ell \in \tnodes $, for some $\ell \geq 2$. We introduce nodes $m_1, \ldots , m_{\ell -1}$ labeled with $\alabel (n_0)$, delete the edges from $n_0$ to $n_1, \ldots , m_\ell $ and add edges $m_i$ to $n_i$ and $m_{i+1}$, for all $i \in \interv {1}{\ell -2}$ then edges from $m_{\ell -1}$ to $n_{\ell -1}$ and $n_\ell $. This step is repeated for each node with more than two children in $\tree $. \item [(\ref {it4:reduced-td})] For each node $n$ with children $n_1, n_2$, we relabel add nodes $n_1', n_2'$ with $\alabel (n) = \alabel (n_1')=\alabel (n_2')$, delete the edges from $n$ to $n_1,n_2$, and add edges from $n$ to $n_1',n_2'$ as well as edges from $n_1'$ to $n_1$ and from $n_2'$ to $n_2$. \item [(\ref {it6:reduced-td})] For each node $n \in \tnodes $, we add $k+1-\cardof {\alabel (n)}$ fresh elements from $\universeGeneral $. Note that the added elements appear exactly once in the tree decomposition, and, hence, the conditions of a tree decomposition remain satisfied. \item [(\ref {it5:reduced-td})] Let $n$ be a node whose only child is $n'$ with $\alabel (n) \neq \alabel (n')$. If $\alabel (n)$ and $\alabel (n')$ differ by more than one element we add a chain of nodes between $n$ and $n'$ such that the sets of labels of two neighboring nodes in the chain differ by exactly one element. \end {compactitem} \par \qed } \par We show that the set $\sidsem {\apred _k()}{\twsid {k}}$ contains only structures of treewidth at most $k$. Let $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure such that $(\universeGeneral ,\struc ) \models _{\twsid {k}} \apred _k()$. By rule (\ref {rule:gen-top}), there exists a store $\store $ with $\store (x_i) = \vertex _i$, for all $1 \le i \le k+1$, and a structure $(\universeGeneral ,\struc ') \in \strucof {\signature ,\domsymb }$ that agrees with $(\universeGeneral ,\struc )$ on $\signature $ such that $(\universeGeneral ,\struc ') \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$ and $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\vertex _1,\ldots ,\vertex _{k+1}}$. The rest of the proof goes by induction on the definition of the satisfaction relation for \slr \ and is given in the following lemma: \par \begin {lemma} \label {lem:sid-implies-tree-decomposition} Let $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure and $\store $ be a store, such that $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred (x_1,\ldots ,x_{k+1})$ and $\store (x_i) \not \in \struc (\domsymb )$, for all $i \in \interv {1}{k+1}$. Then, there exists a reduced tree decomposition $\tree = (\tnodes ,\tedges ,r,\alabel )$ of $\struc $, such that $\twof {\tree }=k$, $\alabel (r)=\set {\store (x_1),\ldots ,\store (x_{k+1})}$ and $\alabel (n) \subseteq \struc (\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\}$, for all $n \in \tnodes $. \end {lemma} \proof { We prove the claim by induction on the number of rule applications. The claim clearly holds for the base case, by rule (\ref {rule:gen-rel}). We now consider the rule (\ref {rule:gen-comp}), i.e., we assume that $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred (x_1,\ldots ,x_{k+1}) * \apred (x_1,\ldots ,x_{k+1})$. Then, there exist structures $(\universeGeneral _1,\struc _1)$ and $(\universeGeneral _2,\struc _2)$, such that $(\universeGeneral _i,\struc _i,) \models ^\store _{\twsid {k}} \apred (x_1,\ldots ,x_{k+1})$, for $i = 1,2$ and $(\universeGeneral _1,\struc _1) \scomp (\universeGeneral _2,\struc _2) = (\universeGeneral ,\struc )$. We note that the latter implies that $\struc _1(\domsymb ) \cap \struc _2(\domsymb ) = \emptyset $ ($\dagger $). We now apply the inductive hypothesis and obtain reduced tree decompositions $\tree _i$ for $(\universeGeneral _i,\struc _i)$ whose respective roots are labelled by $\{\store (x_1),\ldots ,\store (x_{k+1})\}$ and $\alabel (n) \subseteq \struc (\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\}$, for all nodes $n$ of $\tree _i$ and all $i = 1,2$. We obtain a reduced tree decomposition for $(\universeGeneral ,\struc ) $ by composing $\tree _1$ and $\tree _2$ with a fresh root node labelled by $\{\store (x_1),\ldots ,\store (x_{k+1})\}$. Note that $\tree $ is indeed a tree decomposition,note t because the only elements that may appear in labels of both $\tree _1$ and $\tree _2$ must belong to $\{\store (x_1),\ldots ,\store (x_{k+1})\}$, by ($\dagger $). Clearly, we have $\alabel (n) \subseteq \struc _1(\domsymb ) \cup \struc _2(\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\} = \struc (\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\}$, for all nodes $n$ of the resulting tree decomposition $\tree $. We now consider the rule (\ref {rule:gen-exists}), i.e., we assume that $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \exists y ~.~ \domsymb (y) * \apred (x_1, \ldots ,x_{k+1})[x_i/y]$. Then, there is an element $\vertex \not \in \set {\store (x_1), \ldots , \store (x_{k+1})}$ such that $(\universeGeneral ,\struc ') \models ^{\store [x_i \leftarrow \vertex ])}_{\twsid {k}} \apred (x_1, \ldots ,x_{k+1})$, where the structure $(\universeGeneral ,\struc ')$ agrees with $(\universeGeneral ,\struc )$, except that $\struc (\domsymb ) = \struc '(\domsymb ) \setminus \set {\vertex }$. We now apply the inductive hypothesis and obtain a reduced tree decomposition $\tree _1$ for $\struc '$ whose root is labelled by $(\{\store (x_1),\ldots ,\store (x_{k+1})\} \setminus \{\store (x_i)\}) \cup \{\vertex \}$ and $\alabel (n) \subseteq ((\struc '(\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\}) \setminus \{\store (x_i)\}) \cup \{\vertex \}$, for all nodes $n$ of $\tree _1$ ($\ddagger $). We can now obtain a reduced tree decomposition $\tree $ for $\struc $ by composing $\tree _1$ with an additional root labelled by $\{\store (x_1),\ldots ,\store (x_{k+1})\}$. Note that $\tree $ is indeed a tree decomposition because $\store (x_i) \not \in \alabel (n)$ for every node $n$ of $\tree _1$, because of ($\ddagger $), $\vertex \neq \store (x_i)$ and the assumption that $\store (x_i) \not \in \struc (\domsymb )$. We have $\alabel (n) \subseteq \struc '(\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\} \cup \{\vertex \} = \struc (\domsymb ) \cup \{\store (x_1),\ldots ,\store (x_{k+1})\}$ for all nodes $n$ of the resulting tree decomposition $\tree $. \qed } \par Dually, we prove that any structure of treewidth at most $k$ belongs to $\sidsem {\apred _k()}{\twsid {k}}$. To this end, Lemma \ref {lem:tree-decomposition-implies-sid} below shows that, for each such structure $(\universeGeneral ,\struc )$ there exists a store $\store $, such that $\store (x_i) \not \in \struc (\domsymb )$, for all $i \in \interv {1}{k+1}$ and $\struc \models ^\store _{\twsid {k}} \apred (x_1,\ldots ,x_{k+1})$, and conclude by an application of rule (\ref {rule:gen-top}). \par \begin {lemma}\label {lem:tree-decomposition-implies-sid} Let $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure with $\twof {\struc } \le k$ witnessed by some reduced tree decomposition $\tree =(\tnodes ,\tedges ,r,\alabel )$, with $\alabel (r)=\{\vertex _1,\ldots ,\vertex _{k+1}\}$ and $\struc (\domsymb ) = \bigcup _{n \in \tnodes } \alabel (n) \setminus \{\vertex _1,\ldots ,\vertex _{k+1}\}$, and let $\store $ be a store with $\store (x_i) = \vertex _i$, for all $i \in \interv {1}{k+1}$. Then, $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred _k(x_1, \ldots , x_{k+1})$. \end {lemma} \proof { The proof goes by induction on the structure of $\tree $. The claim clearly holds for the base case, where $\tree $ consists of a single leaf, by rule (\ref {rule:gen-rel}). Consider first the case where the root of $\tree $ has two children. The subtrees $\tree _1$ and $\tree _2$ rooted in the two children induce substructures $(\universeGeneral ,\struc _1)$ and $(\universeGeneral ,\struc _2)$ of $(\universeGeneral ,\struc )$, where $\tuple {v_1, \ldots , v_{\arityof {\arel }}} \in \struc _i(\arel )$ iff $\tuple {v_1, \ldots , v_{\arityof {\arel }}}$ is witnessed by some leaf of $\tree _i$, for $i = 1,2$. Because $\tree $ is a reduced tree decomposition, there is at most one leaf that witnesses a tuple $\tuple {v_1, \ldots , v_{\arityof {\arel }}} \in \struc _i(\arel )$. Hence, we have $\struc = \struc _1 \comp \struc _2$. From the inductive hypothesis we obtain $(\universeGeneral ,\struc _i) \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$, for $i = 1,2$. Hence $(\universeGeneral ,\struc _1 \comp \struc _2) \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1}) * \apred (x_1, \ldots , x_{k+1})$, thus $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$, by rule (\ref {rule:gen-comp}). Consider now the case where the root of $\tree $ has a single child which is not a leaf and consider the subtree $\tree _1$ rooted at this child. Then, there is an element $\vertex \not \in \set {\vertex _1, \ldots , \vertex _{k+1}}$, such that the root of $\tree _1$ is labeled by $\{\vertex _1,\ldots ,\vertex _{i-1},\vertex ,\vertex _{i+1},\ldots ,\vertex _{k+1}\}$. Let $(\universeGeneral ,\struc ')$ be the structure that agrees with $(\universeGeneral ,\struc )$ except that we have $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \{\vertex \}$. By the inductive hypothesis, we obtain $(\universeGeneral ,\struc ') \models ^{\store [x_i \leftarrow \vertex ]}_{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$. Hence, $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \exists y ~.~ \domsymb (y) * \apred (x_1,\ldots ,x_{k+1})[x_i / y]$, thus $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred (x_1,\ldots ,x_{k+1})$, by rule (\ref {rule:gen-exists}). \qed }

The main property of $\twsid {k}$ now follows from Lemmas \ref {lem:sid-implies-tree-decomposition} and \ref {lem:tree-decomposition-implies-sid}:

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}``$\Rightarrow $'' If $(\universeGeneral ,\struc )$ has tree decomposition of width at most $k$, then it also has a reduced tree decomposition $\tree =(\tnodes ,\tedges ,r,\alabel )$ of width $k$, by Lemma~\ref {lemma:reduced-tree-decompositions}. Let $\alabel (r)=\set {\vertex _1, \ldots , \vertex _{k+1}}$ and $\store $ be a store such that $\store (x_i) = \vertex _i$, for all $i \in \interv {1}{k+1}$. By Lemma~\ref {lem:tree-decomposition-implies-sid}, we get that $(\universeGeneral ,\struc ) \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1}) * \domsymb (x_1) * \cdots * \domsymb (x_{k+1})$. Thus, $(\universeGeneral ,\struc ) \models _{\twsid {k}} \apred _k()$, by rule (\ref {rule:gen-top}). \par ``$\Leftarrow $'' By rule (\ref {rule:gen-top}), there exists a store $\store $ with $\store (x_i) = \vertex _i$, for all $1 \le i \le k+1$, and a structure $(\universeGeneral ,\struc ') \in \strucof {\signature ,\domsymb }$ that agrees with $(\universeGeneral ,\struc )$ on $\signature $ such that $(\universeGeneral ,\struc ') \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$ and $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\vertex _1,\ldots ,\vertex _{k+1}}$. By Lemma \ref {lem:sid-implies-tree-decomposition}, there exists a reduced tree decomposition $\tree $ of $(\universeGeneral ,\struc ')$ of width $k$. Thus $\twof {\struc } \leq k$, because $(\universeGeneral ,\struc ')$ agrees with $(\universeGeneral ,\struc )$ on $\signature $ and we have $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\vertex _1,\ldots ,\vertex _{k+1}}$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Let us consider the structures $(\universeGeneral _1,\struc _1') = \encof {k+1}{(\universeGeneral _1,\struc _1)}{\store }$ and $(\universeGeneral _2,\struc _2') = \encof {k+1}{(\universeGeneral _2,\struc _2)}{\store }$. In order to apply glueing, we will now consider two structures isomorphic to $(\universeGeneral _1,\struc _1')$ and $(\universeGeneral _1,\struc _2')$, respectively. We note that $\Dom {\struc _1'} \cap \Dom {\struc _2'} \subseteq \{\struc _2'(\acst _{\ncst _1}),\ldots ,\struc _2'(\acst _{\ncst +k+1})\}$ because of the assumption $\Rel {\struc _1} \cap \Rel {\struc _2} \subseteq \{\store (x_1),\ldots ,\store (x_{k+1})\}$). We further note that $\struc _1'(\acst _{\ncst _i}) = \struc _2'(\acst _{\ncst _i})$, for all $i \in \interv {1}{\ncst +k+1}$, because $\struc _1$ and $\struc _2$ are compatible and the interpretation of the additional constants $\acst _{\ncst +1},\ldots ,\acst _{\ncst +k+1}$ has been chosen w.r.t. the same store $\store $. Because $\universeGeneral _1$ and $\universeGeneral _2$ are infinite (recall that we require all universes to be infinite), we can now choose some partitioning $\universeGeneral _1' \uplus \universeGeneral _2' = \universeGeneral _1 \cup \universeGeneral _2$, such that $\universeGeneral _1'$ and $\universeGeneral _2'$ are infinite, $\Dom {\struc _1'} \subseteq \universeGeneral _1$ and $\Dom {\struc _2'} \setminus \{\struc _2'(\acst _1),\ldots ,\struc _2'(\acst _{\ncst +k+1})\} \subseteq \universeGeneral _2$. We can now choose a structure $(\universeGeneral _2,\struc ''_2)$ that is isomorphic to $(\universeGeneral _2,\struc _2')$ and that agrees with $(\universeGeneral _2,\struc _2')$ except for $\acst _1,\ldots \acst _{\ncst +k+1}$, whose interpretation is chosen as $\struc ''_2(\acst _1), \ldots , \struc ''_2(\acst _{\ncst +k+1}) \in \universeGeneral _2 \setminus (\Dom {\struc _1'} \cup \Dom {\struc _2'})$. Then, $(\universeGeneral _1',\struc _1')$ [resp. $(\universeGeneral _2',\struc ''_2)$] is isomorphic to $(\universeGeneral _1,\struc _1')$ [resp. $(\universeGeneral _2,\struc _2')$]. In particular, they have the same type, i.e., $\typeof {r}{\universeGeneral _1',\struc _1'} = \typeof {r}{\universeGeneral _1,\struc _1'}$ and $\typeof {r}{\universeGeneral _2',\struc ''_2} = \typeof {r}{\universeGeneral _2,\struc _2'}$. Moreover, we have that $\glueof {(\universeGeneral _1',\struc _1')}{(\universeGeneral _2',\struc ''_2)}$ and $\encof {k+1}{(\universeGeneral _1,\struc _1) \scomp (\universeGeneral _2,\struc _2)}{\store }$ are isomorphic. In particular, they have the same type, i.e., $$\typeof {r}{\encof {k+1}{(\universeGeneral _1,\struc _1) \scomp (\universeGeneral _2,\struc _2)}{\store }} = \\ \typeof {r}{\glueof {(\universeGeneral _1',\struc _1')}{(\universeGeneral _2',\struc ''_2)}}.$$ We compute: \vspace *{-.5\baselineskip } \[\begin {array}{l} \typeof {r}{\encof {k+1}{(\universeGeneral _1,\struc _1) \scomp (\universeGeneral _2,\struc _2)}{\store }} = \\ \typeof {r}{\glueof {(\universeGeneral _1',\struc _1')}{(\universeGeneral _2',\struc ''_2)}} = \\ \absglueof {\typeof {r}{\universeGeneral _1',\struc _1'}}{\typeof {r}{\universeGeneral _2',\struc ''_2}} = \\ \absglueof {\typeof {r}{\universeGeneral _1,\struc _1'}}{\typeof {r}{\universeGeneral _2,\struc '_2}} = \\ \absglueof {\typeof {r}{\encof {k+1}{(\universeGeneral _1,\struc _1)}{\store }}}{\typeof {r}{\encof {k+1}{(\universeGeneral _2,\struc _2)}{\store }}} \end {array}\]\end{proof}

We prove that the set $\sidsem {\apred _{k,\phi }()}{\twformsid {k}{\phi }}$ contains only structures whose $\qrof {\phi }$-type contains $\phi $, i.e., models of $\phi $. Let $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure such that $(\universeGeneral ,\struc ) \models _{\twformsid {k}{\phi }} \apred _{k,\phi }$. By rule (\ref {rule:ref-top}), there exists a store $\store $ with $\store (x_i) = \vertex _i$, for all $1 \le i \le k+1$, and a structure $(\universeGeneral ,\struc ') \in \strucof {\signature ,\domsymb }$ that agrees with $(\universeGeneral ,\struc )$ on $\signature $ such that $(\universeGeneral ,\struc ') \models ^\store _{\twformsid {k}{\phi }} \apred (x_1, \ldots , x_{k+1})$ and $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\vertex _1,\ldots ,\vertex _{k+1}}$. The rest of the proof uses induction on the definition of the satisfaction relation for \slr : \par \begin {lemma}\label {lem:refined-SID-is-sound} Let $k\geq 1$ be an integer, $\phi $ be an \mso \ sentence, $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure and $\store $ be a store such that $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^\atype (x_1, \ldots , x_{k+1})$, $\store (x_i) \not \in \struc (\domsymb )$ for all $i \in \interv {1}{k+1}$, and $\store (x_i) \neq \store (x_j)$ for all $i \neq j$. Then, $\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \atype $. \end {lemma} \proof { We prove the claim by induction on the number of rule applications. The claim clearly holds for the base case, by a rule of type (\ref {rule:ref-rel}). We now consider a rule of type (\ref {rule:ref-comp}), i.e., we have $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^{\atype _1}(x_1, \ldots , x_{k+1}) * \apred ^{\atype _2}(x_1, \ldots , x_{k+1})$, such that $\atype = \absglueof {\atype _1}{\atype _2}$. Then, there are structures $(\universeGeneral _1,\struc _1)$ and $(\universeGeneral _2,\struc _2)$ with $(\universeGeneral _i,\struc _i) \models ^\store _{\twformsid {k}{\phi }} \apred ^{\atype _i}(x_1, \ldots , x_{k+1})$, for $i = 1,2$, and $\struc _1 \comp \struc _2 = \struc $. By the inductive hypothesis, we have that $\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral _i,\struc _i)}{\store }} = \atype _i$, for $i=1,2$. Because every derivation of $\twformsid {k}{\phi }$ is also a derivation of $\twsid {k}$, obtained by removing the type annotations from the rules in $\twformsid {k}{\phi }$, we get that $(\universeGeneral _i,\struc _i) \models ^\store _{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$, for $i=1,2$. By Lemma~\ref {lem:sid-implies-tree-decomposition} we have that $\Rel {\struc _i} \subseteq \struc _i(\domsymb ) \cup \{\store (x_1), \ldots , \store (x_{k+1})\}$, for $i=1,2$. Since $\struc = \struc _1 \comp \struc _2$, we have that $\struc _1(\domsymb ) \cap \struc _2(\domsymb ) = \emptyset $. We compute \vspace *{-.5\baselineskip } \[\begin {array}{l} \typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \\ \absglueof {\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral _1,\struc _1)}{\store }}}{\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral _2,\struc _2)}{\store }}} = \\ \absglueof {\atype _1}{\atype _2} = \atype \end {array}\] \par \vspace *{-.5\baselineskip }\noindent by Lemma~\ref {lemma:abstract-glue}. We now consider rules of type (\ref {rule:ref-exists}), i.e., we have $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \exists y ~.~ \domsymb (y) * \apred ^{\atype _1}(x_1, \ldots ,x_{k+1})[x_i/y]$, for some $i \in \interv {1}{k+1}$, such that $\atype = \absglueof {\absfgcst {\ncst +i}(\atype _1)}{\rho _i}$ for the type $\rho _i$ of some structure $\astruc \in \strucof {\set {\acst _{\ncst +i}}}$ with a singleton universe and $\astruc \Models \domsymb (\acst _{\ncst +i})$. Then, there is an element $\vertex \in \universeGeneral $, such that $(\universeGeneral ,\struc ') \models ^{\store [x_i \leftarrow \vertex ]}_{\twformsid {k}{\phi }} \apred ^{\atype _1}(x_1, \ldots ,x_{k+1})$, where the structure $(\universeGeneral ,\struc ')$ agrees with $(\universeGeneral ,\struc )$, except that $\domsymb $ does not hold for $\vertex $ in $(\universeGeneral ,\struc ')$. By the inductive hypothesis, $\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]}} = \atype _1$. Because every derivation of $\twformsid {k}{\phi }$ is also a derivation of $\twsid {k}$, obtained by removing the type annotations from the rules in $\twformsid {k}{\phi }$, we get that $(\universeGeneral ,\struc ') \models ^{\store [x_i \leftarrow \vertex ]}_{\twsid {k}} \apred (x_1, \ldots , x_{k+1})$. By Lemma~\ref {lem:sid-implies-tree-decomposition} we have that $\Rel {\struc '} \subseteq \struc '(\domsymb ) \cup \{\store (x_1), \ldots , \store (x_{k+1})\} \setminus \{\store (x_i)\} \cup \{u\}$. Because of $\store (x_i) \neq u$ (due to the assumption $\store (x_i) \not \in \struc (\domsymb )$) and because of $\store (x_i) \neq \store (x_j)$ for all $i \neq j$, we get that $\encof {k+1}{(\universeGeneral ,\struc )}{\store } = \glueof {\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}{\astruc '}$, where $\astruc ' \in \strucof {\set {\acst _{\ncst +i}}}$ is the structure with singleton universe $\{\store (x_i)\}$ and $\astruc ' \Models \domsymb (\acst _{\ncst +i})$. Because $\astruc $ is isomorphic to $\astruc '$, we obtain: \[\begin {array}{l} \typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \\ \typeof {\qrof {\phi }}{ \glueof {\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}{\astruc '}} = \\ \absglueof {\typeof {\qrof {\phi }}{\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}}{\typeof {\qrof {\phi }}{\astruc '}} = \\ \absglueof {\absfgcst {\ncst +i}(\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]}})}{\typeof {\qrof {\phi }}{\astruc }} = \\ \absglueof {\absfgcst {\ncst +i}(\atype _1)}{\rho _i} = \atype \end {array}\] \qed } \par Second, we prove the dual statement, namely that each structure of treewidth at most $k$ and of $\qrof {\phi }$-type that contains $\phi $ must belong to $\sidsem {\apred _{k,\phi }()}{\twformsid {k}{\phi }}$. To this end, Lemma \ref {lem:refined-SID-is-complete} below shows that, for each structure $(\universeGeneral ,\struc )$ of treewidth at most $k$ and $\qrof {\phi }$-type $\atype $, there exists a store $\store $, such that $\store (x_i) \not \in \struc (\domsymb )$, for all $i \in \interv {1}{k+1}$ and $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^\atype (x_1,\ldots ,x_{k+1})$, and we conclude by an application of the rule (\ref {rule:ref-top}): \par \begin {lemma}\label {lem:refined-SID-is-complete} Let $k\geq 1$ be an integer, $\atype $ be some $r$-type, $(\universeGeneral ,\struc ) \in \strucof {\signature ,\domsymb }$ be a structure of treewidth $\twof {\struc } \le k$, witnessed by some reduced tree decomposition $\tree =(\tnodes ,\tedges ,r,\alabel )$, and $\store $ be a store with $\alabel (r)=\{\store (x_1),\ldots ,\store (k+1)\}$ and $\store (x_i) \neq \store (x_j)$ for all $i \neq j$, such that $\struc (\domsymb ) = \bigcup _{n \in \tnodes } \alabel (n) \setminus \{\vertex _1,\ldots ,\vertex _{k+1}\}$ and $\typeof {r}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \atype $. Then, we have $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^\atype (x_1, \ldots , x_{k+1})$. \end {lemma} \proof { The proof proceeds by induction on the structure of $\tree $. Clearly the claim holds for the base case, by a rule of type (\ref {rule:ref-rel}). For the inductive step, we assume first that the root of $\tree $ has two children. The subtrees $\tree _1$ and $\tree _2$ rooted in the two children induce substructures $(\universeGeneral ,\struc _1)$ and $(\universeGeneral ,\struc _2)$ of $(\universeGeneral ,\struc )$, where $\tuple {v_1, \ldots , v_{\arityof {\arel }}} \in \struc _i(\arel )$ if and only if $\tuple {v_1, \ldots , v_{\arityof {\arel }}}$ is witnessed by some leaf of the respective subtree. Because $\tree $ is a reduced tree decomposition, there is at most one leaf that witnesses a tuple $\tuple {v_1, \ldots , v_{\arityof {\arel }}} \in \struc _i(\arel )$. Hence, we have $\struc = \struc _1 \comp \struc _2$. Because the only elements that can appear as labels in $\tree _1$ and $\tree _2$ are $\store (x_1),\ldots ,\store (x_{k+1})$ (as these are the labels of the root of the tree decomposition), we get that $\Rel {\struc _1} \cap \Rel {\struc _2} \subseteq \set {\store (x_1),\ldots ,\store (x_{k+1})}$. Let $\atype _i = \typeof {r}{\encof {k+1}{(\universeGeneral ,\struc _i)}{\store }}$, for $i=1,2$. From the inductive hypothesis, we obtain $(\universeGeneral ,\struc _i) \models ^\store _{\twformsid {k}{\phi }} \apred ^{\atype _i}(x_1, \ldots , x_{k+1})$, for $i=1,2$. Let $\atype \isdef \absglueof {\atype _1}{\atype _2}$. By Lemma~\ref {lemma:abstract-glue}, we obtain: \[\begin {array}{l} \typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc _1) \scomp (\universeGeneral ,\struc _2)}{\store }} = \\ \absglueof {\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc _1)}{\store }}}{\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc _2)}{\store }}} = \\ \absglueof {\atype _1}{\atype _2} = \atype \end {array}\] Hence, we now get that $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^\atype (x_1, \ldots , x_{k+1})$, by a rule of type (\ref {rule:ref-comp}). We now assume that the root of $\tree $ has a single child which is not a leaf. We consider the subtree $\tree _1$ rooted at this child. Then, there is an element $\vertex \not \in \set {\store (x_1), \ldots , \store (x_{k+1})}$, such that the root of $\tree _1$ is labeled by $\set {\store (x_1), \ldots ,\store (x_{i-1}), \vertex ,\store (x_{i+1}), \ldots , \store (x_{k+1})}$. Let $\atype _1 \isdef \typeof {r}{\encof {k+1}{(\universeGeneral ,\struc )}{\store [x_i \leftarrow \vertex ]}}$ and let $(\universeGeneral ,\struc ')$ be the structure that agrees with $(\universeGeneral ,\struc )$ except that we have $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \{\vertex \}$. By the inductive hypothesis, we obtain that $(\universeGeneral ,\struc ') \models ^{\store [x_i \leftarrow \vertex ]}_{\twformsid {k}{\phi }} \apred ^{\atype _1}(x_1, \ldots , x_{k+1})$. Let $\atype \isdef \absglueof {\absfgcst {\ncst +i}(\atype _1)}{\rho _i}$ for the type $\rho _i$ of the structure $\astruc \in \strucof {\set {\acst _{\ncst +i}}}$ with singleton universe $\{\store (x_i)\}$ and $\astruc \Models \domsymb (\acst _{\ncst +i})$. Because of $\store (x_i) \neq u$ and $\store (x_i) \neq \store (x_j)$ for all $i \neq j$, we have $\encof {k+1}{(\universeGeneral ,\struc )}{\store } = \glueof {\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}{\astruc }$. We compute: \[\begin {array}{l} \typeof {r}{\encof {k+1}{(\universeGeneral ,\struc )}{\store }} = \\ \typeof {r}{ \glueof {\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}{\astruc }} = \\ \absglueof {\typeof {r}{\fgcst {\ncst +i}(\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]})}}{\typeof {r}{\astruc }} = \\ \absglueof {\absfgcst {\ncst +i}(\typeof {r}{\encof {k+1}{(\universeGeneral ,\struc ')}{\store [x_i \leftarrow \vertex ]}})}{\typeof {r}{\astruc }} = \\ \absglueof {\absfgcst {\ncst +i}(\atype _1)}{\rho _i} = \atype \end {array}\] \par \vspace *{-.5\baselineskip }\noindent Hence, we get that $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \exists y ~.~ \domsymb (y) * \apred _\tau (x_1, \ldots ,x_{k+1})[x_i/y]$, i.e., that $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \apred ^\atype (x_1, \ldots , x_{k+1})$ by a rule of type (\ref {rule:ref-exists}). \qed }

The main property of the $\twformsid {k}{\phi }$ SID is proved below, by an application of Lemma \ref {lem:refined-SID-is-sound} and \ref {lem:refined-SID-is-complete}:

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}``(\ref {it2:kform-sid}) $\Rightarrow $ (\ref {it1:kform-sid})'' Since $\twof {\universeGeneral ,\struc } \leq k$, there exists a reduced tree decomposition $\tree =(\tnodes ,\tedges ,r,\alabel )$ of width $k$, by Lemma~\ref {lemma:reduced-tree-decompositions}. Let $\store $ be a store such that $\alabel (r) = \set {\store (x_1), \ldots , \store (x_{k+1})}$ and $\store (x_i) \neq \store (x_j)$ for all $i \neq j \in \interv {1}{k+1}$. Let $(\universeGeneral ,\struc ')$ be the structure that agrees with $(\universeGeneral ,\struc )$ on $\signature $, and for which $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\store (x_1),\ldots ,\store (x_{k+1})}$. We observe that $\encof {k+1}{(\universeGeneral ,\struc ')}{\store } = (\universeGeneral ,\struc )$. Thus, we obtain $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \domsymb (x_1) * \ldots * \domsymb (x_{k+1}) * \apred ^\atype (x_1,\ldots ,x_{k+1})$, by Lemma~\ref {lem:refined-SID-is-complete}, for $\atype \isdef \typeof {\qrof {\phi }}{\universeGeneral ,\struc } = \typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc ')}{\store }}$. Since, moreover, we have assumed that $(\universeGeneral ,\struc ) \Models \phi $, we have $\phi \in \atype \isdef \typeof {\qrof {\phi }}{\universeGeneral ,\struc }$. Then, we obtain $(\universeGeneral ,\struc ) \models _{\twformsid {k}{\phi }} \apred _{k,\phi }()$, by a rule of type (\ref {rule:ref-top}). \par ``(\ref {it1:kform-sid}) $\Rightarrow $ (\ref {it2:kform-sid})'' Since $(\universeGeneral ,\struc ) \models _{\twformsid {k}{\phi }} \apred _{k,\phi }()$, there exists a store $\store $ with $\store (x_i) \neq \store (x_j)$ for all $i \neq j \in \interv {1}{k+1}$, such that $(\universeGeneral ,\struc ) \models ^\store _{\twformsid {k}{\phi }} \domsymb (x_1) * \ldots * \domsymb (x_{k+1}) * \apred ^\atype (x_1, \ldots , x_{k+1})$, for some type $\atype $ with $\phi \in \atype $, by a rule of type (\ref {rule:ref-top}). Let $(\universeGeneral ,\struc ')$ be the structure that agrees with $(\universeGeneral ,\struc )$ on $\signature $, and for which $\struc '(\domsymb ) = \struc (\domsymb ) \setminus \set {\store (x_1),\ldots ,\store (x_{k+1})}$. We observe that $\encof {k+1}{(\universeGeneral ,\struc ')}{\store } = \struc $. By Lemma~\ref {lem:refined-SID-is-sound}, we obtain $\typeof {\qrof {\phi }}{\encof {k+1}{(\universeGeneral ,\struc ')}{\store }} = \atype $. With $\encof {k+1}{(\universeGeneral ,\struc ')}{\store } = (\universeGeneral ,\struc )$ and $\phi \in \atype $ we then obtain $(\universeGeneral ,\struc ) \Models \phi $. Moreover, we have $\twof {\universeGeneral ,\struc } \leq k$, by Lemma \ref {lemma:k-sid}, because each derivation of $(\universeGeneral ,\struc ') \models _{\twformsid {k}{\phi }} \apred _{k,\phi }()$ corresponds to a derivation of $(\universeGeneral ,\struc ) \models _{\twsid {k}} \apred _{k}()$, obtained by removing the type annotations from the rules in $\twformsid {k}{\phi }$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}We consider the $r$-round MSO Ehrenfeucht-Fra\"{i}ss\'{e} game: In every round, Spoiler picks a vertex $\vertex $ or a set of vertices $\vertexSet $ in $\astruc $ or $\astruc ^{2^r}$ and Duplicator answers with a vertex or a set of vertices in the other structure. Duplicator wins iff after $r$-rounds the substructures induced by the selected vertices are isomorphic. We now sketch a winning strategy for Duplicator (as the argument is standard, we leave the details to the reader): For vertices in $\Dom {\struc }$ the Duplicator plays the same vertices in the respective other structure (this applies to single vertices as well as sets of vertices). For the vertices that do not belong to $\Dom {\struc }$ the Duplicator selects vertices that do not belong to $\Dom {\struc }$ in the other structure such that the selected vertices belong to the same subsets played in the previous rounds; care has to be taken for the involved cardinalities, if playing in $\astruc ^{2^r}$ the Duplicator limits himself to at most $2^{r-k-1}$ vertices that belong to any combination of previously played subsets or the complement of these subsets, where $k$ is the number of previously played rounds; this choice is sufficient such that after $r$-rounds the substructures induced by the selected vertices are isomorphic.\end{proof}

